Human-in-the-Loop Task and Motion Planning for Imitation Learning

Imitation learning from human demonstrations can teach robots complex manipulation skills, but is time-consuming and labor intensive. In contrast, Task and Motion Planning (TAMP) systems are automated and excel at solving long-horizon tasks, but they are difficult to apply to contact-rich tasks. In this paper, we present Human-in-the-Loop Task and Motion Planning (HITL-TAMP), a novel system that leverages the benefits of both approaches. The system employs a TAMP-gated control mechanism, which selectively gives and takes control to and from a human teleoperator. This enables the human teleoperator to manage a fleet of robots, maximizing data collection efficiency. The collected human data is then combined with an imitation learning framework to train a TAMP-gated policy, leading to superior performance compared to training on full task demonstrations. We compared HITL-TAMP to a conventional teleoperation system -- users gathered more than 3x the number of demos given the same time budget. Furthermore, proficient agents (75\%+ success) could be trained from just 10 minutes of non-expert teleoperation data. Finally, we collected 2.1K demos with HITL-TAMP across 12 contact-rich, long-horizon tasks and show that the system often produces near-perfect agents. Videos and additional results at https://hitltamp.github.io .

==> A-video.tex <==
\section{Supplemental Video Overview}
\label{app:video}

The supplemental video contains:
\begin{enumerate}
    \item Real-World \sysName policies on Tool Hang, Coffee Broad, Stack Three, and Coffee.
    \item \sysName dataset trajectories visualized across the 9 simulated tasks. The red border indicates human control (and the lack of one indicates TAMP control).
    \item \sysName initial state distribution visualizations across the 9 simulated tasks.
\end{enumerate}
